Planck 2015 results. XX. Constraints on inflation

We present the implications for cosmic inflation of the Planck measurements of the cosmic microwave background (CMB) anisotropies in both temperature and polarization based on the full Planck survey. The Planck full mission temperature data and a first release of polarization data on large angular scales measure the spectral index of curvature perturbations to be $n_\mathrm{s} = 0.968 \pm 0.006$ and tightly constrain its scale dependence to $d n_s/d \ln k =-0.003 \pm 0.007$ when combined with the Planck lensing likelihood. When the high-$\ell$ polarization data is included, the results are consistent and uncertainties are reduced. The upper bound on the tensor-to-scalar ratio is $r_{0.002} < 0.11$ (95% CL), consistent with the B-mode polarization constraint $r< 0.12$ (95% CL) obtained from a joint BICEP2/Keck Array and Planck analysis. These results imply that $V(\phi) \propto \phi^2$ and natural inflation are now disfavoured compared to models predicting a smaller tensor-to-scalar ratio, such as $R^2$ inflation. Three independent methods reconstructing the primordial power spectrum are investigated. The Planck data are consistent with adiabatic primordial perturbations. We investigate inflationary models producing an anisotropic modulation of the primordial curvature power spectrum as well as generalized models of inflation not governed by a scalar field with a canonical kinetic term. The 2015 results are consistent with the 2013 analysis based on the nominal mission data.

==> Tables/table_r_extended_rounded.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{ccccc}
\noalign{\hrule\vskip 2pt}
\noalign{\hrule\vskip 3pt}
Extended model, & Parameter & \Planck\ TT+lowP & \Planck\ TT+lowP & \Planck\ TT,TE,EE \\
$\Lambda$CDM+$r$+ & & +lensing & +BAO & +lowP \\
\noalign{\hrule\vskip 2pt}
%\hline
%Inflationary & $\ln B_{0X}$ & $\Delta \chi^2$ \\
%Model & & \\
%\hline
\multirow{2}{*}{+general reionization} & $r$ & $r < 0.11$ & $r < 0.10$ & $< 0.10$ \\

& $n_{\mathrm{s}}$ & $0.975 \pm 0.006$ & $0.971 \pm 0.005$ & $0.968 \pm 0.005$ \\
%$r_{002}$ &  \textcolor{red}{$< X$} & \textcolor{red}{$< X$} &\textcolor{red}{$0.9681$} \\
\noalign{\hrule\vskip 2pt}
& $r$ &  $< 0.14$ & $< 0.12$ & $< 0.11$ \\
+$N_\mathrm{eff}$ & $n_{\mathrm{s}}$
& $0.977^{+0.016}_{-0.017}$ & $0.972 \pm 0.009$ & $0.964 \pm 0.010$ \\
%$r_{002}$ &  $< 0.137$ & $< 0.113$ & $< 0.100$ \\
\noalign{\vskip 2pt}
& $N_\mathrm{eff}$  &  $3.24^{+0.30}_{-0.35}$ & $3.19 \pm 0.24$ &
$3.02^{+0.20}_{-0.21}$ \\
\noalign{\hrule\vskip 2pt}
& $r$  & $< 0.14$ & $< 0.12$ & $<0.12$ \\
+$Y_\mathrm{He}$
& $n_{\mathrm{s}}$ & $0.975 \pm 0.007$ & $0.973 \pm 0.009$ & $0.969 \pm 0.008$ \\
%$r_{002}$ &  $< 0.142$ & < 0.117 & $< 0.112$ \\
& $Y_\mathrm{He}$  & $0.258 \pm 0.022$ & $0.257 \pm 0.022$ & $0.252 \pm 0.014$ \\
%& $Y_\mathrm{He}$  & $0.2577^{+0.0218}_{-0.0217}$ & $0.2574^{+0.0218}_{-0.0217}$ & $0.2524^{+0.0136}_{-0.0135}$ \\
\noalign{\hrule\vskip 2pt}
& $r$  &  $< 0.11$ & $< 0.11$ & $< 0.11$\\
+$m_\nu$ & $n_\mathrm{s}$ & $0.963 \pm 0.007$ & $0.967 \pm 0.005$ & $0.962 \pm 0.005$ \\
%$r_{002}$ &  $< 0.103$ & $< 0.101$ & $< 0.104$ \\
& $m_\nu$ & $< 0.67$ & $< 0.21$ &  $< 0.58$ \\
\noalign{\hrule\vskip 2pt}
& $r$ & $< 0.15$  & $r < 0.11$ & $< 0.15$\\
+$\Omega_K$ & $n_{\mathrm{s}}$ & $0.971 \pm 0.007$
& $0.971 \pm 0.007$ & $0.969 \pm 0.005$ \\
%$r_{002}$ &  $< 0.143$ & \textcolor{red}{$< X$} & $< 0.145$ \\
& $\Omega_K$ & $-0.008^{+0.010}_{-0.008}$  & $-0.001 \pm 0.003$ &
$-0.045^{+0.016}_{-0.020}$ \\
\noalign{\hrule\vskip 2pt}
& $r$  & $< 0.14$ & $< 0.11$ & $< 0.12$ \\
+$w$&
$n_{\mathrm{s}}$ & $0.969 \pm 0.006$ & $0.967 \pm 0.006$ & $0.966 \pm 0.005$ \\
%$r_{002}$ &  $< 0.130$ & $< 0.104$ & $< 0.115$ \\
& $w$ & $-1.46^{+0.20}_{-0.40}$ & $-1.02^{+0.08}_{-0.07}$ & $-1.57^{+0.17}_{-0.37}$ \\
\noalign{\hrule\vskip 2pt}
\multirow{4}{*}{+$\Omega_K$+$d n_\mathrm{s}/d \ln k$} & $r$ & $< 0.20$  & $< 0.18$ & $< 0.19$ \\

& $n_{\mathrm{s}}$ & $0.971 \pm 0.007 $ & $0.969 \pm 0.007$ & $0.969 \pm 0.005$ \\
%$r_{002}$ &  $< 0.210$ & $< 0.197$ & \textcolor{red}{$< X$} \\
& $d n_\mathrm{s}/d \ln k$ & $-0.006 \pm 0.009$ &
$-0.013 \pm 0.009$ & $-0.004 \pm 0.008$ \\
& $\Omega_K$ & $-0.006^{+0.010}_{-0.009}$ & $-0.001 \pm 0.003$ &
$-0.043^{+0.011}_{-0.020}$ \\
\noalign{\hrule\vskip 2pt}
\multirow{4}{*}{+$N_\mathrm{eff}$+$m_\mathrm{eff}$}& $r$ & $r < 0.14$ & $r < 0.13$ & $< 0.12$ \\

& $n_{\mathrm{s}}$ & $0.980^{+0.010}_{-0.014}$ & $0.978^{+0.008}_{-0.011}$ &
$0.968^{+0.006}_{-0.008}$ \\
%$r_{002}$ &  \textcolor{red}{$< X$} & \textcolor{red}{$< X$} &\textcolor{red}{$0.9681$} \\
& $m_\mathrm{eff}$ & $< 0.27$ & $<0.21$ & $<0.83$ \\
& $N_\mathrm{eff}$ & $< 3.45$ & $<3.73$ & $<3.47$ \\
\hline
\end{tabular}
\end{center}
\caption{Constraints on extensions of the $\Lambda$CDM+$r$ cosmological
model for \Planck\ TT+lowP+lensing, \Planck\ TT+lowP+BAO, and \Planck\ TT,TE,EE+lowP. 
For each model we quote 68\,\% CL, unless 95\,\% CL upper bounds are reported. 
%bounds on $r$, $n_{\mathrm{s}}$, additional parameters.
%{\color{red} [JL: I suspect that this is not true, and that the above table may feature sometimes
%95\%CL and sometimes 68\%CL bounds. For instance, the error bar on $n_s$ for $\Lambda$CDM+r+YHe and $\Lambda$CDM+r+mnu using TT+lowP+lensing is suspiciously small for 95\%CL (and actually even for 68\%)]}
}
\label{tab:r_extended}
\end{table*}



==> Tables/wl_table.tex <==

\begin{table}[tmb]                 % table* is a two-column table.  Drop the * for one column.
\begin{center}
  \begingroup
  \newdimen\tblskip \tblskip=5pt
%\caption{%
%Prior for moveable knot positions. 
%The $\PR$ positions are distributed in a log-uniform manner across a wide range. 
%The $k$ positions are also log-uniformly distributed 
%across the entire range needed by {\tt CosmoMC} and are sorted so that ${k_1<\ldots<k_{\Nknots}}$. 
%When we marginalize over the number of knots, $\Nknots$, we assume a uniform prior between 2 and 10.
%  }
  \label{tab:P_k_priors}                            % Label goes here.
  \nointerlineskip
  \vskip -3mm
  \footnotesize
  \setbox\tablebox=\vbox{
    \newdimen\digitwidth
    \setbox0=\hbox{\rm 0}
    \digitwidth=\wd0
    \catcode`*=\active
    \def*{\kern\digitwidth}
    %
    \newdimen\signwidth
    \setbox0=\hbox{+}
    \signwidth=\wd0
    \catcode`!=\active
    \def!{\kern\signwidth}
    %
    \halign{%
      \hfil#\hfil&
      \hfil#\hfil\cr
      \noalign{\doubleline}
      Parameter range &
      Prior type
      \cr
      \noalign{\vskip 3pt\hrule\vskip 5pt}
      $10^{-4}\,\mathrm{Mpc}^{-1} = k_1< k_2 < \ldots < k_{\Nknots} = 0.3\,\mathrm{Mpc}^{-1}$ &
      log uniform (sorted)
      \cr
      $ 2 < \ln\left(10^{10}\Pknotj{1}\right), \ldots ,\ln\left(10^{10}\Pknotj{{\Nknots}}\right) < 4 $  &
      log uniform
      \cr
      $2\le \Nknots \le 10 $ &
      integer uniform
      \cr
      \noalign{\vskip 3pt\hrule\vskip 5pt}
      $0.019< \Omega_\mathrm{b} h^2 <0.025$ &
      uniform
      \cr
      $0.095< \Omega_\mathrm{c} h^2 <0.145$ &
      uniform
      \cr
      $1.03< 100\theta_\mathrm{MC} <1.05$ &
      uniform
      \cr
      $0.01< \tau< 0.4$ &
      uniform
      \cr
      \noalign{\vskip 5pt\hrule\vskip 3pt}}}
    \endPlancktable                    % ends one-column \halign
  %\endPlancktablewide                 % ends two-column \halign
  \endgroup
\end{center}
\caption{%
Prior for moveable knot positions.
The $\PR$ positions are distributed in a log-uniform manner across a wide range.
The $k$ positions are also log-uniformly distributed
across the entire range needed by {\tt CosmoMC} and are sorted so that ${k_1<\ldots<k_{\Nknots}}$. 
When we marginalize over the number of knots, $\Nknots$, we assume a uniform prior between 2 and 10. }
\end{table}                        % table* is a two-column table.  Drop the * for one column


